Localized, High-resolution Geographic Representations with Slepian Functions

Geographic data is fundamentally local. Disease outbreaks cluster in population centers, ecological patterns emerge along coastlines, and economic activity concentrates within country borders. Machine learning models that encode geographic location, however, distribute representational capacity uniformly across the globe, struggling at the fine-grained resolutions that localized applications require. We propose a geographic location encoder built from spherical Slepian functions that concentrate representational capacity inside a region-of-interest and scale to high resolutions without extensive computational demands. For settings requiring global context, we present a hybrid Slepian-Spherical Harmonic encoder that efficiently bridges the tradeoff between local-global performance, while retaining desirable properties such as pole-safety and spherical-surface-distance preservation. Across five tasks spanning classification, regression, and image-augmented prediction, Slepian encodings outperform baselines and retain performance advantages across a wide range of neural network architectures.

==> tables/spatio-temporal-main.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Temporal encoding comparison for atmospheric temperature prediction.}
Mean RMSE (mean $\pm$ std across seeds) averaged across eight pressure levels from stratosphere to surface.
\textbf{Bold} indicates best performance, \underline{underline} indicates second best.}
\label{tab:temporal_encoding_condensed}

\vspace{3pt}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
{\small
\begin{tabular}{@{}lc@{}}
\toprule
\textbf{Model} & \textbf{Mean RMSE} \\
\midrule
No Time & 5.703$\pm$0.001 \\
Time Copy & 2.428$\pm$0.018 \\
Triangle & 3.092$\pm$0.003 \\
Monomial & 2.033$\pm$0.178 \\
Legendre & 1.532$\pm$0.285 \\
Fourier & 1.477$\pm$0.128 \\
\midrule
\textcolor{slepianpurple}{DPSS} ($NW{=}15$) & \textbf{1.344$\pm$0.012} \\
\textcolor{slepianpurple}{DPSS} ($NW{=}19$) & \underline{1.357$\pm$0.011} \\
\bottomrule
\end{tabular}
}
\end{table}
